Bounds for spectral projectors on the three-dimensional torus

We study $L^2$ to $L^p$ operator norms of spectral projectors for the Euclidean Laplacian on the torus in the case where the spectral window is narrow. With a window of constant size this is a classical result of Sogge; in the small-window limit we are left with $L^p$ norms of eigenfunctions of the Laplacian, as considered for instance by Bourgain. For the three-dimensional torus we prove new cases of a previous conjecture of the first two authors concerning the size of these norms; we also refine certain prior results to remove $\epsilon$-losses in all dimensions. We use methods from number theory: the geometry of numbers, the circle method and exponential sum bounds due to Guo. We complement these techniques with height splitting and a bilinear argument to prove sharp results. We exposit on the various techniques used and their limitations.

==> OLDBilinearImprovement.tex <==
\section{Removing the $\epsilon$-loss: geodesic focusing case}

\subsection{A bilinear decomposition: the diagonal terms}
We shall follow the approach introduced in \cite{BlairHuangSogge} and adapted to this problem in \cite{Pezzi}, however we shall give a proof that uses Poisson summation instead of microlocal techniques. The two proofs are largely equivalent. 

Previously the following convolution kernel for the mollified projection operator was introduced.

\begin{equation}
    \Phi^\flat(x)=\sum_{k\in \Z{3}}\chi^\flat (k)e^{2\pi ik\cdot x}.
\end{equation}
Where $\chi^\flat(\xi) = \delta^{-2}\chi(\delta^{-1}\cdot)*d\sigma_\la(\xi)$ where $\chi$ is an appropriate compactly supported bump function and $d\sigma_{\la}$ the surface measure on the quadratic form scaled by $\la$. We introduce a partition of unity on the support of $\Phi^{\flat}$. Let $\{\nu\}$ be a maximal $\delta$ separated set on the quadratic form $Q(x) = 1$. Let $\beta_{\nu}(\xi)$ be a partition of unity on $Q(x)=1$ such that each $\beta_\nu$ is compactly supported in a $4\delta$ neighborhood of $\nu$. Furthermore, let $\Tilde{\beta}(\xi)$ be a Littlewood-Paley bump function that is $1$ on the set $[1/2,2]$ and supported in the set $[1/4,4]$. Define the Fourier multiplier $Q_\nu$ by the symbol

\begin{equation}
    q_{\nu}(k)\coloneq \beta_{\nu}(p(k))\Tilde{\beta}(|k|/\la),
\end{equation}
where $p(\xi)$ is the radial projection of $\xi$ to the surface $Q(x)=1$. We have the following result.

\begin{theorem}\label{KNEstThrm}
    Consider the operator $Q_\nu$ and the discrete projection operator $P_{\la,\delta}$. Their composite obeys the following bound.
    \begin{equation}\label{KNEstEqn}
        \lpnorm{Q_{\nu}P_{\la,\delta}f}{p}{\T{3}}\lesssim (\la^{1-\frac{3}{p}}\delta^{1/2}+(\la\delta)^{\frac{1}{2}-\frac{1}{p}})\lpnorm{f}{2}{\T{3}}.
    \end{equation}
\end{theorem}

\begin{proof}
    By a standard application of duality and orthogonality, it suffices to prove \cref{KNEstEqn} with the discrete projection operator replaced with the mollified version. Let $\{\varphi\}$ be a partition of unity on $\T{3}$ such that the support of each $\varphi$ is contained within a sufficiently small ball. The exact size of the ball required depends on the injectivity radius\SMnote{What's an injectivity radius?}\DPnote{A minor technicality. Essentially weird things happen if you take a lattice whose basis vectors are around $\sim \frac{1}{\la}$ or something like that. For the torus, bounded injectivity means the basis vectors are $\sim 1$ in magnitude. I am fine with removing reference to it.} but it will never depend on $\la$. We may replace integration over $\T{3}$ with integration over $\T{3}$ against a $\varphi$ by the triangle inequality. We will analyze the kernel of the operator $Q_\nu \Phi^\flat\coloneq \Phi^\flat_\nu$.

    \begin{equation}
    \Phi^\flat_\nu(x-y)=\sum_{k\in \Z{3}}\chi^\flat (k)q_{\nu}(k)e^{2\pi ik\cdot (x-y)} \coloneq \sum_{k\in\Z{3}}\chi^\flat_{\nu}(k)e^{2\pi i k\cdot (x-y)}.
    \end{equation}

    Following the proof in Section 3, after applying Poisson summation and localization we are left with estimating the following. We have omitted the local term as it enjoys stronger estimates.

    \begin{equation}
    S_{\la,M,x}^{\nu}=\sum_{m\in \Z{3}}\psi(\frac{m-x+y}{M})\widehat{\chi^\flat_{\nu}}(m-x+y).
    \end{equation}
    We will now evaluate $\widehat{\chi^\flat_{\nu}}(m-x+y)$. Clearly 
    
    \begin{equation}
        \widehat{\chi^\flat_{\nu}}(m-x +y) = (\widehat{\chi^\flat}*\hat{q_\nu})(m-x+y).
    \end{equation}
    Expanding this gives
    
    \begin{equation}
        \int_{\R{n}}\widehat{\chi^\flat}(u)\int_{\R{n}}e^{2\pi i(m+y-x-u)\cdot \xi} \beta_{\nu}(p(\xi))\Tilde{\beta}(|\xi|/\la)d\xi du.
    \end{equation}
    We have previously computed that
    
    \begin{equation}
        \widehat{\chi^\flat}(u) = \la^2\delta J(\la u)\hat{\chi}(\delta u).
    \end{equation}
    Where $J$ is the Fourier transform of the surface measure of the sphere. We will apply the stationary phase asymptotic expansion of $J$ but only record the leading terms as the lower order terms are more favorable. We will also omit the sum over $\pm$ and only write.
    
    \begin{equation}
        \la\delta\int_{\R{n}}\frac{e^{\pm i\la|u|}}{|u|}\hat{\chi}(\delta u)\int_{\R{n}}e^{2\pi i(m+y-x-u)\cdot \xi} \beta_{\nu}(p(\xi))\Tilde{\beta}(|\xi|/\la)d\xi du.
    \end{equation}
    We now make the change of variables $z = m+y-u$ to get
    
    \begin{equation}
        \la\delta\int_{\R{n}}\frac{e^{\pm i\la|m+y-z|}}{|m+y-z|}\hat{\chi}(\delta u)\int_{\R{n}}e^{2\pi i(x-z)\cdot \xi} \beta_{\nu}(p(\xi))\Tilde{\beta}(|\xi|/\la)d\xi du.
    \end{equation}
    
    This kernel is a kernel with respect to integration over $\T{3}$. Because of this, we may now reintroduce the partition of unity over $ x\in \T{3}$ given by $\varphi$. Here we are slightly abusing notation by identifying $\T{n}$ with its fundamental domain. By triangle inequality we may then prove bounds with a factor of $\varphi(x)$. Integration by parts in $z$ allows us to then insert another bump function $\tilde{\varphi}(z)$ which is $1$ in a neighborhood of $\phi(z)$. This, after a change of variables $\xi\rightarrow\la\xi$ recovers the form of (6.3.3) from \cite{BlairHuangSogge}. Arguments from that paper give the desired bounds.
        
\end{proof}

Now that we have recovered the key estimate with a fully discrete version of $Q_\nu$, we will quickly review the bilinear decomposition used in \cite{Pezzi} to get sharp results in the geodesic focusing case. We have previously broken up the projector in the following manner.

\begin{equation}
    P_{\la,\delta} = P_0 + \sum_{s}P_s.
\end{equation}
We shall focus on improving the result in the case where the dominant term is $P_{s_{\max}}$. Technically, we shall need some wiggle room. Fix $s_0$ to be close to $s_{max}$ in a manner to be described later. Define

\begin{equation}
    P_{S}\coloneq \sum_{s_0\leq s \leq s_{max}}P_s.
\end{equation}
With a natural definition for $S$. We shall prove that where we have previously shown $P_{s_{\max}}$ obeys the conjecture with $\epsilon$-loss, $P_{S}$ actually obeys the sharp version of the conjecture.

To do so we use the bilinear reduction from \cite{Pezzi}. Specifically, let $\gamma,\gamma'$ be two large caps, namely intersections of of $A_{\la,\delta}$ with cones of by angular aperture $\sim \theta_k$ and angularly separated by $\sim \theta_k$ where $1\gtrsim \theta_k \gtrsim \delta$. Let $P_{\gamma}$ be the projection onto this large cap with the analogous definition for $P_{\gamma'}$ (going forward we will only state definitions for $\gamma$). Then we have the following condition for sharp results.\SMnote{the term 'angular sector' for me has a fixed definition and only refers to a sector in the 2D plane, so I changed the language here, can you confirm this is what was meant?}
\DPnote{This is fine. I will also make sure the new language is consistent.}

\begin{proposition}
    Suppose for some fixed positive $\eta$ we have the following bound for every $1\gtrsim \theta_k \gtrsim \delta$ and every such pair of large caps $\gamma,\gamma'$.

    \begin{equation}\label{bilinearGainEqn}
        \lpnorm{(P_{\gamma}P_{S}f P_{\gamma'}P_{S}f)^{1/2}}{p}{\T{3}}\lesssim (\la\delta)^{\frac{1}{2}-\frac{1}{p}-\eta}(\lpnorm{P_{\gamma}f}{2}{\T{3}}\lpnorm{P_{\gamma'}f}{2}{\T{3}})^{1/2}.
    \end{equation}

    Then \begin{equation}
        \lpnorm{P_S f}{p}{\T{n}}\lesssim (\la\delta)^{\frac{1}{2}-\frac{1}{p}}.
    \end{equation}.
\end{proposition}
We shall only prove \eqref{bilinearGainEqn} when $p=4$ as the result follows by interpolation with either $L^2$ or $L^\infty$ estimates regardless of whether $p$ is smaller or larger than $4$ respectively. The proof of the above proposition is a large portion of \cite{Pezzi}, and so will be omitted here. 

The intuition for the following work is as follows. There are not that many caps in $S$ and so we may freely use the triangle inequality, provided $s_0$ is chosen close to $s_{max}$. Because of our bilinear reduction, any two caps which interact must be transverse, and the $L^4$ norm allows us to compute their interaction explicitly.

\begin{proof}[Proof of \eqref{bilinearGainEqn}]

By the triangle inequality we may write

\begin{equation*}
    \lpnorm{(P_{\gamma}P_{S}f P_{\gamma'}P_{S}f)^{1/2}}{4}{\T{3}}\lesssim \mathbb{E}(\la,\delta)\sup_{\omega,\omega'}\lpnorm{(P_{\omega} f P_{\omega'}f)^{1/2}}{4}{\T{n}}.
\end{equation*}
Where $\mathbb{E}(\la,\delta)$ is a product of powers of $\la$, $\delta$, $2^s$, $2^{s_0}$ with the property that $\mathbb{E}(\la,\delta)\rightarrow C$ as $s_0\rightarrow s_{max}$. We also take $\omega,\omega'$ to be caps with non-empty intersection with $\gamma,\gamma'$ respectively.

We choose to measure in the $L^4$ norm not because it is critical for decoupling in $n=3$, but bcause it lets us tie the norm to the geometry of the lattice points in the caps. Because $\omega,\omega'$ have near the maximum number of lattice points, the lattice points must be contained on $2$ dimensional affine spaces. After applications of Parseval's identity and Cauchy-Schwarz, one gets the following bound.

\begin{equation}
    \lpnorm{(P_{\omega} f P_{\omega'}f)^{1/2}}{4}{\T{n}}\lesssim M^{1/4}(\lpnorm{P_{\omega}f}{2}{\T{3}}\lpnorm{P_{\omega'}f}{2}{\T{3}})^{1/2}.
\end{equation}
Where

\begin{equation}
    M\coloneq \sup_{(b,b')\in (\omega,\omega')}|\{(a,a')\in \omega \times \omega': a + a' = b + b'\}|.
\end{equation}
There is a slight abuse of notation where we have conflated $\omega$ and $\omega'$ with the lattice points contained in $\omega$ and $\omega'$ in the previous notation. 

As the large caps\SMnote{change "arcs" to "large caps"} $\gamma,\gamma'$ are transverse by at least $\delta$, the normal vectors of the affine spaces that contain the lattice points in $\omega,\omega'$ must also be transverse. Obviously $a+a' = b + b'$ if and only if $a-b = b'-a'$. This shows that for a fixed $(b,b')$, the set of $(a,a')$ that satisfy the condition must each lie on a 1 dimensional affine subspace. As selecting $a$ fixes $a'$ and vice versa, this gives that 
\begin{equation*}
    M\lesssim (\la\delta)^{1/2},
\end{equation*}
as lattice points have $O(1)$ separation distance and the the length of the longest line in a cap is $\lesssim (\la\delta)^{1/2}$.

When $p =4$ we are trying to beat a bound of $(\la\delta)^{\frac{1}{4}}$. The above work proves, after taking the supremum over $\omega,\omega'$ that

    \begin{equation}\label{bilinearGainEqn}
        \lpnorm{(P_{\gamma}P_{S}f P_{\gamma'}P_{S}f)^{1/2}}{4}{\T{3}}\lesssim E(\la,\delta)(\la\delta)^{\frac{1}{8}}(\lpnorm{P_{\gamma}f}{2}{\T{3}}\lpnorm{P_{\gamma'}f}{2}{\T{3}})^{1/2}.
    \end{equation}

We have also used the inequality $\lpn{P_\omega}{2}\leq \lpn{P_{\gamma}}{2}$ for every $\omega\subset \gamma$. Taking $s_{0}$ sufficiently close to $s_{max}$ gives the result at $p=4$. The rest follows by interpolation with either $L^2$ or $L^\infty$ estimates.
\end{proof}







==> OLDHeightSplitting2.tex <==
\section{Removing the $\eps$-loss: Point focusing case}
We have already shown that the operator $P_{\lambda,\delta}$ obeys the conjecture with $\epsilon$ loss when $\delta\gtrsim \la^{-\frac{1}{2}}$. In this section we shall sharpen this result by removing the $O_\eps(\la^\eps)$ factor when $\delta\gtrsim \la^{-\frac{1}{2}+\kappa}$ for a fixed positive $\kappa$. We shall do so by following the argument in \cite{BlairHuangSogge}.

\begin{proposition}\label{P0prop} For any positive definite quadratic form $Q$,
\begin{equation}\label{sharpP0Eqn}
        \lpnorm{P_{\lambda,\delta} f}{p}{\T{3}}\lesssim_{\kappa} \la^{1-\frac{3}{p}}\delta^{1/2}\lpnorm{f}{2}{\T{3}}
\qquad \mbox{if  $\delta \geq \lambda^\kappa [ \lambda^{2-\frac p2} + \lambda^{-\frac 12}]$}.
    \end{equation}
\end{proposition}
For the proof we wish to combine the height decomposition used by Blair-Huang-Sogge in \cite{BlairHuangSogge} and the caps decomposition as earlier.

\begin{proof} \underline{Step 1: mollifying the operator.}
Defining $\mathcal{S}_\lambda$ to be the ellipsoid $\{ x, \; Q(x)=\la^2\}$ and $\dd \sigma_{\mathcal{S}_\lambda}$ to be the superficial measure on this ellipsoid, we let
$$
\phi_{\lambda,\delta}(x) = \delta^{-2} \phi (\delta^{-1} \cdot) * \dd \sigma_{\mathcal{\mathcal{S}_\lambda}},
$$\DPnote{We use $\phi$ here instead of $\chi$, I assume because of the cap cutoffs taking that symbol. Do we want to use $\phi$ in the previous sections and the latter?}
where $\phi$ is a smooth and nonnegative function with compact support. In this way $\|\phi_{\lambda,\delta}\|_{L^1(\mathbb R^3)}\approx \delta \lambda^2$ and $\phi_{\lambda,\delta}$ is supported within $O(\delta)$ of the ellipsoid.  The square root of this symbol gives the Fourier multiplier $P^{\sharp}_{\lambda,\delta}$:
$$
P^{\sharp}_{\lambda,\delta} = \sqrt{\phi_{\lambda,\delta}}(D), \qquad 
(P^{\sharp}_{\lambda,\delta})^2 = \phi_{\lambda,\delta}(D).
$$
Since $\chi_{\lambda,\delta}(k)>c>0$ if $|Q(k) - \lambda| <c \delta$, for a sufficiently small constant $c$, it suffices to prove that the statement of the theorem holds if $P_{\lambda,\delta}$ is replaced by $P_{\lambda,\delta}^\sharp$.

Recall that the Fourier transform (on $\mathbb{R}^d$) of $\dd \sigma_1$ is such 
$$
m (\xi) = \widehat{\dd \sigma_1}(\xi) \qquad \mbox{satisfies} \qquad |m(\xi)| \lesssim \langle \xi \rangle^{-1}
$$
Since $\dd \sigma_\lambda = \lambda^{-1} \dd \sigma_1(\la^{-1}\cdot)$, we have
$$
\widehat{\phi_{\lambda,\delta}}(\xi) = \lambda^2 \delta m(\lambda \xi) \widehat{\phi}(\delta \xi).
$$
This formula will be crucial in the following to obtain bounds on the kernels of various operators.

\medskip

\noindent  \underline{Step 2: decompositions into caps and heights.}
Similar to $P^s_{\lambda,\delta}$, we define $P^{\sharp,s}_{\lambda,\delta}$. Then, we decompose $P^{\sharp}_{\lambda,\delta}$ into two pieces: $P_{\operatorname{avg}}$ gathering all caps with average (or slightly greater) number of points, and $P_{\operatorname{rem}}$ gathering the remaining caps, which therefore contain many more points than average:
$$
P_{\operatorname{avg}} = \sum_{2^s < \lambda^{1} \delta^2} \chi_s(D), \qquad  P_{\operatorname{rem}} = \sum_{2^s > \lambda^{1+\eta} \delta^2} \chi_s(D).
$$
We need to bound $P^{\sharp}_{\lambda,\delta} P_{\operatorname{avg}}$ and
$P^{\sharp}_{\lambda,\delta} P_{\operatorname{rem}}$.
Since $\eta >0$, the latter operator can be easily disposed of by the proof of Theorem~\ref{thm:caps}, which gives a nonzero power saving in $\lambda$ compared to the conjectured $\lambda^{1 - \frac 3p} \delta^{\frac 12}$. Therefore we turn to the former operator.\SMnote{I would like to double check or reword this} \PGnote{I tried to explain a bit more - what do you think?}

In order to prove that $P^{\sharp}_{\lambda,\delta} P_{\operatorname{avg}}$ has an operator norm $\lesssim \lambda^{1-\frac 3p} \delta^{\frac 12}$ from $L^2$ to $L^p$, it suffices to show that
$$
\| P^{\sharp}_{\lambda,\delta} f \|_{L^p} \lesssim \lambda^{1-\frac 3p} \delta^{\frac 12}
$$
for $f$ such that
$$
\| f \|_{L^2} = 1 \quad \mbox{and} \quad P_{\operatorname{avg}} f = f,
$$
which we assume henceforth.

Finally, the last decomposition is to split the torus into large and small height:
\begin{equation} \label{defA-A+}
\begin{split}
& A_- = \{x\in \T{3} : | P^{\sharp}_{\lambda,\delta} f(x)| < C_0 (\la\delta^{-1})^{\frac{1}{2}}\} \\
& A_+= \{x\in \T{3} : | P^{\sharp}_{\lambda,\delta} f(x)| \geq C_0 (\la\delta^{-1})^{\frac{1}{2}}\}
\end{split}
\end{equation}

\medskip

\noindent \underline{Step 3: small height.} On the one hand, the $L^\infty$ norm of $P^{\sharp}_{\lambda,\delta} f$ on $A_-$ is bounded by the very definition of $A_-$
\begin{equation}\label{P0smallheightsbound}
        \lpnorm{P^{\sharp}_{\lambda,\delta} f}{\infty}{A_-}\lesssim (\la\delta^{-1})^{\frac{1}{2}}.
    \end{equation}
On the other hand, its $L^4$ norm on $A_-$ can be estimated by \eqref{Pfew} to give\SMnote{What's the argument here?} \PGnote{added the ref}
$$ 
\lpnorm{P^{\sharp}_{\lambda,\delta}  f}{4}{A_-} \leq \lpnorm{P^{\sharp}_{\lambda,\delta}f}{4}{\T{3}}
= \lpnorm{ P^{\sharp}_{\lambda,\delta} P_{\operatorname{avg}} f}{4}{\T{3}} \lesssim_\epsilon \la^{\epsilon} \la^{\frac 14 }\delta^{\frac 12}.
$$

Interpolating between these two norms yields\SMnote{I need to think briefly what happened to $\epsilon$, but I guess there should just be an $\epsilon $ in the penultimate term}\DPnote{Over the subset $A_-,$ there is a power saving in the $L^\infty$ norm that overrides the $\epsilon$ loss from decoupling. It is why the $\kappa>0$ wiggle room is necessary.} \PGnote{added the $\epsilon$ loss}
\begin{equation}\label{P0holderbound}
\begin{split}
\lpnorm{P^{\sharp}_{\lambda,\delta} f}{p}{A_-}&  \leq \lpnorm{P^{\sharp}_{\lambda,\delta} f}{\infty}{A_-}^{\frac{p-4}{p}}
\| P^{\sharp}_{\lambda,\delta} f \|_{L^4(A_-)}^{\frac{4}{p}} \\
& \leq \lambda^{\frac 4p \epsilon}\lambda^{\frac 12 - \frac 1p} \delta^{-\frac 12 + \frac 4p} \leq \lambda^{1 - \frac 3p} \delta^{\frac 12},
\end{split}
\end{equation}
where the last inequality is a consequence of $\delta>\lambda^{-\frac 12+\kappa}$.

\medskip

\noindent \underline{Step 4: large height.} By duality and self-adjointness of $ P^{\sharp}_{\lambda,\delta}$, there exists  $g\in L^{p'}(A_+)$ with $L^{p'}$ norm $1$ such that
$$
\| P^{\sharp}_{\lambda,\delta} f \|_{L^p(A_+)} = \int \mathbf{1}_{A_+} \cdot P^{\sharp}_{\lambda,\delta} f \cdot g \dd x \leq \| P^{\sharp}_{\lambda,\delta} \mathbf{1}_{A_+} g \|_{L^2}.
$$
Therefore,
\begin{align*}
\| P^{\sharp}_{\lambda,\delta} f \|_{L^p(A_+)}^2 & \leq \int P^{\sharp}_{\lambda,\delta} \mathbf{1}_{A_+} g \cdot \overline{P^{\sharp}_{\lambda,\delta} \mathbf{1}_{A_+} g} \dd x 
= \int (P^{\sharp}_{\lambda,\delta})^2 \mathbf{1}_{A_+} g \cdot  \overline{\mathbf{1}_{A_+} g} \dd x,
\end{align*}
where we again used that the projection operator is self-adjoint. At this point, we split $(P^{\sharp}_{\lambda,\delta})^2$ into a "local" part $L_{\lambda}$ and a "global" part $G_{\lambda,\delta}$:
$$
(P^{\sharp}_{\lambda,\delta})^2 = L_\lambda + G_{\lambda,\delta}, \qquad L_\lambda = \delta (P^{\sharp}_{\lambda,1})^2, \qquad G_{\lambda,\delta} = (P^{\sharp}_{\lambda,\delta})^2 - \delta (P^{\sharp}_{\lambda,1})^2.
$$
From the above, we see that we need to estimate
$$
\int L_\la (\mathbf{1}_{A_+}\cdot g(x))\overline{(g\cdot \mathbf{1}_{A_+})(x)} dx + \int G_\la (\mathbf{1}_{A_+}\cdot g(x))\overline{(g\cdot \mathbf{1}_{A_+})(x)} dx = I + II.
$$

The local piece is easily estimated. Indeed, H\"older's inequality and Sogge's universal estimates lead to the bound 
\begin{align*}
|I| \leq \| L_\lambda (g\cdot \mathbf{1}_{A_+}) \|_{L^p} \| g\cdot \mathbf{1}_{A_+}\|_{L^{p'}} \leq \| L_{\lambda} \|_{L^{p'} \to L^{p}} \| g\cdot \mathbf{1}_{A_+}\|_{L^{p'}}^2 \lesssim \delta\lambda^{2-\frac{6}{p}}.
\end{align*}

In order to bound $II$, we need to estimate the $L^\infty$ norm of the convolution kernel of $G_{\lambda,\delta}$. By Poisson summation, it equals
$$
G_{\lambda,\delta}(x) = \sum_{n \in \mathbb{Z}^3} \lambda^2 \delta \left[ \widehat{\phi}(\delta( x+n))) - \widehat{\phi}(x+n) \right] m(\lambda(x+n)).
$$
Observe that \SMnote{This seems true but not totally trivial, I get $\lambda^2\delta \langle x^{-1}\rangle^{-1} \langle \lambda x\rangle^{-1}$ and then I have to do three cases}
\PGnote{I added the sentence between parentheses - is it enough, or do you want me to say more?}
$$
\left| \lambda^2 \delta \left[ \widehat{\phi}(\delta x) - \widehat{\phi}(x) \right] m(\lambda x) \right|
\lesssim
\lambda \delta \langle x \rangle^{-1},
$$
(which can be seen by distinguishing the cases $|x| < \frac 1 \lambda$, $\frac 1 \lambda < |x| < 1$, and $|x|>1$)
and that it decays rapidly for $x \gg \frac{1}{\delta}$. This gives the  bound 
$$
\| G_\lambda(x) \|_{L^\infty} \leq C_1 \lambda \delta^{-1},
$$
for a constant $C_1>0$. This allows to bound $II$ using H\"older's inequality, the definition of $g$, and the definition of $A_+$. 
\begin{align*}
    |II|&\leq C_1 \la\delta^{-1}\lpn{\mathbf{1}_{A_{+}}\cdot g}{1}^2 \leq C_1(\la\delta^{-1}) (\lpn{\mathbf{1}_{A_+}}{p}\lpn{g}{p'})^2\\
    &\leq C_1C_0^2 (\la\delta^{-1})((\la\delta^{-1})^{-1/2}\lpnorm{P^\sharp_{\lambda,\delta} f}{p}{A_{+}})^2\leq  \frac{1}{4}\lpnorm{ P^\sharp_{\lambda,\delta} f}{p}{A_{+}}^2;
\end{align*}
here, we chose $C_0$ so that $C_1 C_0^2\leq \frac{1}{4}$.

Combining with our bound for $I$ gives 

\begin{equation*}
    \lpnorm{P^\sharp_{\lambda,\delta} f}{p}{A_+}^2\leq C\delta \la^{2-\frac{6}{p}} + \frac{1}{4}\lpnorm{P^\sharp_{\lambda,\delta} f}{p}{A_+}^2,
\end{equation*}
which finally yields the desired estimate!
\end{proof}


==> OLD_HeightSplitting.tex <==
\section{Removing the $\eps$-loss: Point focusing case}
We have already shown that the operator $P_0$ obeys the conjecture with $\epsilon$ loss when $\delta\gtrsim \la^{-\frac{1}{2}}$. In this section we shall sharpen this result by removing the $O_\eps(\la^\eps)$ factor when $\delta\gtrsim \la^{-\frac{1}{2}+\kappa}$ for a fixed positive $\kappa$. A similar decomposition to the one we applied to the $P_s$ operators could be used here but it does not improve our result.

\PGnote{PG: in this section, $P_0$ means $\sum_s P^s_{\lambda,\delta}$ with $2^s<$ average number of points... Am I right?}

\begin{proposition}\label{P0prop} Let $\T{3}$ be an arbitrary torus.  Then if $\delta\gtrsim \la^{-\frac{1}{2}+\kappa}$ for some fixed positive $\kappa$, we have the sharp bound

    \begin{equation}\label{sharpP0Eqn}
        \lpnorm{P_0 f}{p}{\T{3}}\lesssim_{\kappa} \la^{1-\frac{3}{p}}\delta^{1/2}\lpnorm{f}{2}{\T{3}}.
    \end{equation}
\end{proposition}
For the proof we wish to combine the height decomposition used by Blair-Huang-Sogge in \cite{BlairHuangSogge} and the specific estimates involving caps used by Demeter-Germain \cite{DemeterGermain} and Germain-Myerson \cite{GermainMyerson1}. We will now introduce a smooth approximation to $P_{\la,\delta}$. Let $\rho$ be a Schwartz class function on $\R{}$ such that $\rho(0)=1$ and $\supp\hat{\rho}\subset \{t\in \R{}: |t|\in (c/2,c)\}$ for some sufficiently small constant $c$. Then by the spectral theorem we can define the operator

\begin{equation}
    \rho(\delta^{-1}(\la - P))f  = \sum_{j=0}^\infty \rho(\delta^{-1}(\la - \la_j))E_jf,
\end{equation}
where $P =\sqrt{-\Delta_{\T{3}}}$ and $E_jf$ is the Fourier projection onto the $j$-th eigenspace. This approximates $P_{\la,\delta}$ and crucially the two operators commute. We will prove sharp estimates in line with the conjecture for the composite $\rho P_{0}$ over all of $\T{3}$ largely for technical reasons. The approach of Blair--Huang--Sogge works with the smoothed out $\rho$ operator while the approach of Germain--Myerson prefers the discrete operator $P_{\la,\delta}$. Considering the composite $\rho P_0$ allows for consistency when we combine techniques from these two different camps, and it is equivalent bounding $P_0$ by the following lemma.

\begin{lemma}\label{orthogDualityP0Lemma}
    For any number $C$, suppose we have the bound 

    \begin{equation*}
        \lpnorm{\rho P_0 f}{p}{\T{3}}\lesssim C(\la,\delta) \lpnorm{f}{2}{\T{3}}.
    \end{equation*}
    Then we have the bound

    \begin{equation*}
        \lpnorm{P_0 f}{p}{\T{3}}\lesssim C(\la,\delta) \lpnorm{f}{2}{\T{3}}.
    \end{equation*}
\end{lemma}

\begin{proof}
    This a standard application of orthogonality and duality. By duality and the assumption of the lemma we have
    
    \begin{equation}\label{P0duality}
        \lpnorm{\rho P_0 f}{2}{\T{3}}\leq C\lpnorm{f}{p'}{\T{3}}
    \end{equation}
    Orthogonality gives the following expression for the square of the left hand side of \eqref{P0duality}

    \begin{equation*}
        \sum_{i=0}^{\infty}\rho(\delta^{-1}(\la-\la_j))^2\lpn{E_j P_0f}{2}^2.
    \end{equation*}
    Where $E_j$ is the projection onto the $j$-th eigenspace. By assumption the Fourier transform of $\rho$ is compactly supported, so $\rho$ experiences rapid decay. Separate the $\la_j$ into dyadic groups $\Lambda_j$ defined by $\la_j\in \Lambda_j$ if and only if $\delta^{-1}(\la-\la_j)\sim 2^j$ with the usual definition of $\Lambda_0$. As $\rho$ is bounded the triangle inequality shows the frequencies in $\Lambda_0$ can be bounded by $P_{\la,c\delta}$ for some $c$. For the frequencies in $\Lambda_j$ as simple computation using the Weyl law and the rapid decay shows the local term dominates up to a multiplied constant..
\end{proof}

The reason for considering the composite $\rho P_0$ is that we wish to split $\T{3}$ into two sets. On one set we will want to work with the smoothed out operator and on the other we will want to work with the discrete projection. Splitting based on the composite allows us to work with two sets that partition the torus. Specifically, consider the set

\begin{equation*}
        A_+ \coloneq \{x\in \T{3} : |\rho P_{0}f(x)| \geq C(\la\delta^{-1})^{\frac{1}{2}}\},
\end{equation*}
for some constant $C$. Define $A_{-} \coloneq \T{3}\setminus A_+$. 


We shall take a moment to digest the implications of this decomposition in the context of the torus. In the windows Blair-Huang-Sogge considered for general manifolds with non-positive curvature, the height threshold $(\la \delta^{-1})^{\frac{1}{2}}$ always represents an improvement over the trivial $L^\infty$ norm. In the context of the torus, this is only an improvement over $\la\delta^{1/2}$ if $\delta > \la^{-\frac{1}{2}+\kappa}$ for an arbitrarily small but fixed $\kappa$. This is a manifestation of $A_{\la,\delta}$ containing a degenerate number of lattice points when compared to a general $1$-separated set. In this range we can use the below argument to estimate $\rho P_{0}f$ restricted to $A_+$ and obtain the sharp bound that arises in the point focusing regime. Once we have dealt with the large heights, our improved $L^\infty$ norm on $A_-$ allows us to conclude easily. If $\delta$ is taken to be smaller then $A_+$ would be an empty set and we do not get an improved bound for $A_-$.

In the following proposition $P_{0}$ plays no role and the result holds for arbitrary $f$. We only include it to align with the small height estimate where this situation will be reversed; we will work exclusively with $P_{0}$ on $A_{-}$ and ignore $\rho$ except in the fact it enables this decomposition.

\begin{proposition}\label{largeHeightsP0prop}
    Let $P_{\la,\delta}f$ be the discrete Fourier projection of $f$ onto $A_{\la,\delta}$ and $\rho$ its smoothed out approximation. Let $P_0$ be the projection defined in the previous subsection. Let 
    \begin{equation*}
        A_+ = \{x\in \T{3} : |\rho P_{0}f(x)| \geq C(\la\delta^{-1})^{\frac{1}{2}}\}.
    \end{equation*}

    For some $C>0$ to be selected later. Then 
    
    \begin{equation}\label{largeHeightBound}
        \lpnorm{\rho P_{0}f}{p}{A_+}\lesssim \lambda^{1 - \frac 3p} \delta^{\frac 12} \lpnorm{f}{2}{\T{3}}.
    \end{equation}
\end{proposition}

\begin{proof}
This is essentially Proposition 6.2 from \cite{BlairHuangSogge}. Using duality and $\lpn{P_{0}f}{2}\leq 1$ we have

\begin{equation*}
        \lpnorm{\rho P_{0}f}{p}{A_+}^2 \leq \int L_\la (1_{A_+}\cdot g(x))\overline{(g\cdot 1_{A_+})(x)} dx + \int G_\la (1_{A_+}\cdot g(x))\overline{(g\cdot 1_{A_+})(x)} dx = I + II.
    \end{equation*}
    For some appropriate $g\in L^{p'}(A_+)$ with $L^{p'}$ norm $1$. Here we have that 

    \begin{equation*}
        L_\la = \frac{\delta}{2\pi}\int a(t)\hat{\Psi}(\delta t)e^{it\la}e^{it\sqrt{-\Delta_g}} dt,
    \end{equation*}
    where $\Psi = \rho_\la^2, a(t)$ is a bump function centered at 0, and $e^{it\sqrt{-\Delta_g}}$ is the half-wave propagator. $G_\la$ is the same but with $a(t)$ replaced by $1-a(t)$. We call $L_\la$ a local operator and $G_\la$ a global operator. 

    The local operator obeys the following bound by Sogge's universal estimates, see \cite{Sogge}, and scaling.

    \begin{equation*}
        \lpn{L_\la}{L^{p'}(\T{3})\rightarrow L^{p}(\T{3})}\lesssim \delta\la^{2-\frac{6}{p}}.
    \end{equation*}
    Which allows us to estimate via H\"older

    \begin{align*}
        |I|&\leq \lpn{L_\la (g\cdot 1_{A_+})}{p}\lpn{g\cdot 1_{A_+}}{p'}\\
        &\leq \delta\la^{2-\frac{6}{p}}\bigPara{\lpn{g\cdot 1_{A_+}}{p'}}^2\\
        &\leq \delta\la^{2-\frac{6}{p}}.
    \end{align*}

For $G_\la$ we introduce a dyadic cutoff in time which let's us write the kernel of $G_{\la,j}$ as 

\begin{equation*}
    G_{\la,j}(x,y) = \frac{\delta}{2\pi}\int_{-\infty}^\infty (1-a(t))\beta(t/2^j)\hat{\Psi(\delta t)}e^{-t\la}e^{-t\sqrt{-\Delta_{\T{3}}}}(x,y)dt.
\end{equation*}
Where $e^{-itP}(x,y)$ is the kernel of the half wave propagator. By Euler's formula the principle of non-stationary phase we may replace the operator $e^{-it\sqrt{-\Delta_{\T{3}}}}$ by $\cos(\sqrt{-\Delta_{\T{3}}})$. This is because the above kernel with $e^{it\sqrt{-\Delta_{\T{3}}}}$ enjoys rapid decay. After lifting to the universal cover of $\T{3}$ we have

\DPnote{I will take $k_l = k$ for now, its exact representation depends on the normalization for $\T{3}$ we want to use in the paper. I will go through and adjust all constants and such later.}

\PGnote{I suggest we try and use the normalization I wrote down in the first few paragraphs of the article. Everything is not consistent yet, but I will be trying to homogenize things.}
\begin{equation*}
    (\cos(\sqrt{-\Delta_{\T{3}}}))(x,y) = \sum_{k\in \Z{3}}\cos(\sqrt{-\Delta_{\R{3}}})(x,(y+k_l)).
\end{equation*}
Where $k_l$ indexes the universal cover. Therefore, up to lower order errors we may consider the kernel

\begin{align}\label{GapproxKernelDef}
    \Tilde{G}_{\la,j}(x,y)&\coloneq \sum_{k\in \Z{3}}\frac{\delta}{2\pi}\int_{-\infty}^\infty\beta(|t|/2^j)\hat{\Psi(\delta t)}e^{-t\la}\cos(\sqrt{-\Delta_{\R{3}}})(x,(y+j_l))dt\\
    &= \sum_{k\in \Z{3}}K(x,y+k_l).
\end{align}

Our goal is to show $\lpn{\Tilde{G}_{\la,j}}{1\rightarrow \infty} = O(\delta \la2^{2j})$. After summing over all $1\lesssim 2^j \lesssim \delta^{-1}$, this will imply the necessary bound for $G_{\la}$. We see that one term in the sum in \cref{GapproxKernelDef} is given by the following up to lower order terms after appealing to the Hadamard parametrix.

\begin{equation*}
    \frac{\delta}{\pi}(2\pi)^{-3}\int \int e^{i\la t}e^{i\langle x-y,\xi \rangle}(\cos(t|\xi|))\beta(|t|/2^j)\hat{\Psi}(\delta t)dt d\xi.
\end{equation*}

The only region that significantly contributes is when $|x-y|\sim 2^j$. Regions where $|x-y|$ is larger do not contribute by finite speed of propagation, and regions where $|x-y|$ is smaller do not contribute by non-stationary phase. Using Lemma 5.13 in \cite{Sogge} this term can be expressed as

\begin{equation*}
    \sum_{\pm}\delta \la 2^{-j}e^{\pm i\la|x-y|}a_{\pm}(\la,|x-y|)+O(\la^{-N}).
\end{equation*}
\DPnote{the $a_{\pm}$ functions should basically be a cutoff times $\frac{1}{|x-y-k|}$ which is what allows one to use exponential sum estimates, I will track down a direct argument at some point. this aligns it with $S_{\la,M,x}$ more or less. Exponential sum estimates improve the bound in the square torus case.}

We are trying to estimate

\begin{equation*}
    \Tilde{G}_{\la,j}(x,y)=\sum_{k\in \Z{3}}K(x,y+k_l).
\end{equation*}
There are $2^{jn}$ points $k_l$ such that $|x-y|\sim 2^j$ for a fixed $x$ and $y$. By summing over all such choices we get

\begin{equation*}
    |\Tilde{G}_{\la,j}(x,y)| = O(\delta \la 2^{2j}).
\end{equation*}

This implies $\lpn{G_{\la}}{1\rightarrow \infty}\lesssim \la \delta^{-1}$ after summing over $2^j$. This immediately bounds $II$ using H\"older's, the definition of $g$, and the definition of $A_+$. Here we must take the $C$ such that $|\rho_\la P_0f|\geq C(\la\delta^{-1})^{1/2}$ on $A_+$ so that $C_0C^2\leq \frac{1}{4}$.

\begin{align*}
    |II|&\leq C_0 \la\delta^{-1}\lpn{1_{A_{+}}\cdot g}{1}^2 \leq C_0(\la\delta^{-1}) (\lpn{1_{A_+}}{4}\lpn{g}{4/3})^2\\&\leq C_0C^2 (\la\delta^{-1})((\la\delta^{-1})^{-1/2}\lpnorm{\rho_\la P_{0} f}{p}{A_{+}})^2\leq  \frac{1}{4}\lpnorm{\rho_\la P_{0} f}{p}{A_{+}}^2,
\end{align*}

\PGnote{I cannot follow this sequence of inequalities, can you explain what you use for the second and third $\leq$?}

Combining with our bound for $I$ gives 

\begin{equation*}
    \lpnorm{\rho_{\la} P_0 f}{p}{A_+}^2\leq C\delta \la^{2-\frac{6}{p}} + \frac{1}{4}\lpnorm{\rho_{\la} P_0 f}{p}{A_+}^2.
\end{equation*}

Which yields

\begin{equation*}
    \lpnorm{\rho_{\la} P_0 f}{p}{A_+}\lesssim \la^{1-\frac{3}{p}}\delta^{1/2}.
\end{equation*}
Recalling that $||f||_2=1$, this gives the correct $L^2\rightarrow L^p$ bound for $\rho_{\la} P_0$.

\end{proof}

\begin{corollary}
    Suppose $\T{3}$ is the square torus. Then one may improve the the bound of $|\Tilde{G}_{\la,j}(x,y)|$ which improves the range of $\delta$ that $P_0$ obeys the sharp estimates.
\end{corollary}

\begin{proof}
    Reviewing the previous proof, we wish to prove $L^1 \rightarrow L^\infty$ bounds for the operators $\Tilde{G}_{\la,j}$. We did this by lifting to the universal cover and writing

    \begin{equation*}
        \Tilde{G}_{\la,j}(x,y) = \sum_{k\in \Z{3}}K_{\la,\delta,j}(x,y+k_l).
    \end{equation*}
    Where each $K_{\la,\delta,j}(x,y+k_l)$ term is of the form

    \begin{equation}
       \delta \la 2^{-j}e^{\pm i\la|x-y-k_l|}a(\la,|x-y-k_l|).
    \end{equation}
    Where we have dispensed with the rapidly decreasing errors and with the sum over $\pm$. It is known that $a(\la,|x-y-k_l|)$ is uniformly bounded and that we have restricted to $2^j\sim |x-y-k_l|$. Because of this we can, after summing over $k$, write this term as 

    \begin{equation*}
        \sum_{k\in \Z{3}}\la \delta \frac{e^{\pm i\la|x-y-k_l|}}{|x-y-k_l|}a(\la,|x-y-k_l|).
    \end{equation*}

    Pointwise estimates for this sum that are better than the trivial ones lead to a better bound for $\Tilde{G}_{\la,j}(x,y)$, which allows for a more aggressive height splitting.    
\end{proof}
\DPnote{This may run into trouble as the presence of the amplitude $a(\la,\cdot)$ may mess up the exponential sum bounds. In this case it may make sense to try height splitting on the discrete projector, so this would involve rewriting this prove but using the estimates in section 3. If one restricts to $P_0$ there should be a better interpolation. }

To finish the proof of \Cref{P0prop} we only need to prove the same estimate on $A_-$ as $\T{3}=A_+\cap A_-$.

\begin{proposition}\label{smallHeightsP0}
    Let $P_{\la,\delta}f$ be the discrete Fourier projection of $f$ onto $A_{\la,\delta}$ and $\rho$ its smoothed out approximation. Let $P_0$ be the projection defined in the previous subsection. Let 
    \begin{equation*}
        A_- = \{x\in \T{3} : |P_{0}\rho f(x)| \leq C(\la\delta^{-1})^{\frac{1}{2}}\}.
    \end{equation*}

    For some $C>0$ to be selected later. When $\delta\gtrsim \la^{-\frac{1}{2}+\kappa}$ we have
    
    \begin{equation}\label{largeHeightBound}
        \lpnorm{P_{0}\rho f}{p}{A_-}\lesssim \mathbb{E}_{1,gain}(\la,\delta)\lpnorm{f}{2}{\T{3}}.
    \end{equation}
\end{proposition}

\begin{proof}
    By H\"older's inequality we have the following

    \begin{equation}\label{P0holderbound}
        \lpnorm{P_{0}\rho f}{p}{A_-} \leq \lpnorm{P_{0}\rho f}{\infty}{A_-}^{\frac{p-4}{p}}\lpnorm{P_{0}\rho f}{4}{A_-}^{\frac{4}{p}}.
    \end{equation}

    By the definition of $A_-$ and $\lpn{f}{2}=1$ we have

    \begin{equation}\label{P0smallheightsbound}
        \lpnorm{P_{0}\rho f}{\infty}{A_-}\lesssim (\la\delta^{-1})^{\frac{1}{2}}\lpnorm{f}{2}{\T{3}}.
    \end{equation}

    By Proposition 5.2 in \cite{GM1} (taking $2^j\lesssim $ in that paper's notation) we have
    \DPnote{This should be changed to a citation for this paper}.


    \begin{equation}\label{P0critexponentbound}
        \lpnorm{P_{0}\rho f}{4}{A_-}\leq\lpnorm{P_{0}\rho f}{4}{\T{3}}\lesssim \la^\epsilon(\la\delta^{1})^{\frac{1}{2}-\frac{1}{4}}\lesssim \la^\epsilon\la^{1/4}\delta^{1/2}.
    \end{equation}

    Plugging \eqref{P0smallheightsbound} and \eqref{P0critexponentbound} into \eqref{P0holderbound} gives the result using that $||f||_2=1$.

    
\end{proof}

